WildIFEval: Instruction Following in the Wild

Recent LLMs have shown remarkable success in following user instructions, yet handling instructions with multiple constraints remains a significant challenge. In this work, we introduce WildIFEval - a large-scale dataset of 7K real user instructions with diverse, multi-constraint conditions. Unlike prior datasets, our collection spans a broad lexical and topical spectrum of constraints, extracted from natural user instructions. We categorize these constraints into eight high-level classes to capture their distribution and dynamics in real-world scenarios. Leveraging WildIFEval, we conduct extensive experiments to benchmark the instruction-following capabilities of leading LLMs. WildIFEval clearly differentiates between small and large models, and demonstrates that all models have a large room for improvement on such tasks. We analyze the effects of the number and type of constraints on performance, revealing interesting patterns of model constraint-following behavior. We release our dataset to promote further research on instruction-following under complex, realistic conditions.

==> figures/categories_and_performance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/heatmap_of_scores_co-occurrences_in_tasks_mean_all_models.png}
    \caption{The effect of co-occurrences on performance. In each row, we see the performance over some constraint, and each column indicates with which constraint type it co-occurred. The values are normalized by the mean performance for each constraint type in general. We only show the scores for tasks with exactly two constraints.}
    \label{fig:score-cooccur}
\end{figure}
